Tensor Completion with BMD Factor Nuclear Norm Minimization

This paper is concerned with the problem of recovering third-order tensor data from limited samples. A recently proposed tensor decomposition (BMD) method has been shown to efficiently compress third-order spatiotemporal data. Using the BMD, we formulate a slicewise nuclear norm penalized algorithm to recover a third-order tensor from limited observed samples. We develop an efficient alternating direction method of multipliers (ADMM) scheme to solve the resulting minimization problem. Experimental results on real data show our method to give reconstruction comparable to those of HaLRTC (Liu et al., IEEE Trans Ptrn Anal Mchn Int, 2012), a well-known tensor completion method, in about the same number of iterations. However, our method has the advantage of smaller subproblems and higher parallelizability per iteration.

==> extra_stuff.tex <==
\begin{document}

%\paragraph{Abstract Mirjeta}
%Tensor completion, that is known to be the task of estimating the missing elements from partially observed data, is ubiquitous in many practical applications. The main task relies on computing a compressed representation of the desired tensor. A recently proposed tensor BM-decomposition (BMD) method has demonstrated an efficient compressibility of third-order spatiotemporal data. In this paper, we formulate a slicewise nuclear norm penalized algorithm to recover a third-order tensor from limited observed samples.We develop an efficient alternating direction method of multipliers (ADMM) scheme to solve the resulting minimization problem. Experimental examples on real-world data are used to illustrate the effectiveness of our method on data recovery with a relatively fast convergence rate.


Data recovery for 2D arrays from partial measurements, referred to as the matrix completion problems, has been well studied in the literature \cite{ cai2010singular,komodakis2006image}. To solve the problem, a common assumption is that the underlying unknown data matrix has low rank, or has approximately low rank. 
The model consists of solving the following optimization problem
\begin{equation*}
    \begin{split}
        \min &\text{ rank}(\M{X})\\
        \text{subject to } &\M{X}_{\Omega} = \M{M}_{\Omega},
    \end{split}
\end{equation*}
where $\M{X} \in \mathbb{R}^{n_1\times n_2}$ is the completed matrix, $\M{M} \in \mathbb{R}^{n_1\times n_2}$ is the incomplete data matrix, and $\Omega$ denotes the indices of the observed entries of $\M{M}$. The equation $\M{X}_{\Omega} = \M{M}_{\Omega}$ means that $\M{X}_{i,j} = \M{M}_{i,j}$ for all $(i,j)\in \Omega$. 
In practice, since the matrix rank is not a convex function, the trace norm of matrices has been used to approximate the rank of matrices which leads to a convex optimization problem \cite{cai2010singular,candes2012exact, candes2010power}. 

%the tensor completion model consists of solving the following optimization problem
%\begin{equation*}
%    \begin{split}
%        \min_{\T{X}} & \text{ rank}(\T{X})\\
%        \text{subject to } & \T{X}_{\Omega} = \T{T}_{\Omega},
%    \end{split}
%\end{equation*}

%The main contributions of this paper are as follows:
%\begin{enumerate}
%    \item We introduce a tractable relaxation of the rank function into our BM-factor tensor rank minimization model.
%    \item We present an efficient alternating direction method of multipliers (ADMM) scheme to solve the proposed problem.
%\end{enumerate}

%\begin{equation}
%    \V{x} = \tvec(\T{X}) = \underset{\begin{array}{c}
%\scriptstyle 1\leq i\leq m\\
%\scriptstyle 1\leq j\leq n
%\end{array}}{\oplus}\V{x}^{(i,j)} \ \in \mathbb{R}^{mnp\times 1},
%\end{equation}
%\begin{equation}
%\V{x}=\tvec(\T{X}) = \left[\begin{array}{c}
%\V{x}^{(1,1)}\\
%\vdots\\
%\V{x}^{(i,j)}\\
%\vdots\\
%\V{x}^{(m,p)}
%\end{array}\right] = 
%\left[\begin{array}{c}
%\sq\left(\T{X}_{1,1,:}\right)\\
%\vdots\\
%\sq\left(\T{X}_{i,j,:}\right)\\
%\vdots\\
%\sq\left(\T{X}_{m,p,:}\right)
%\end{array}\right].
%\end{equation}

%\begin{equation}
%    \V{x} = \tvec(\T{X}) = \underset{i,j}{\oplus} \V{x}^{(i,j)} \quad \forall \ 1\leq i\leq m, 1\leq j \leq n,
%\end{equation}

%and reformulate the problem as follows
%\begin{equation}
%    \begin{split}
%        \min_{\T{X}, \T{A}_i^{(t)}} & \sum_{i=1}^{3}\sum_{t=1}^{\ell} \alpha_{i,t} \|\T{A}_i^{(t)}\|_{*} \\
%        \text{s.t. } &\T{X} = \bmp(\T{A}_1,\T{A}_2,\T{A}_3), \T{X}_{\Omega} = \T{T}_{\Omega},
%    \end{split}
%\end{equation}


\begin{equation}
\min_{\tvec\left(\T{A}_{3}^{\top}\right)}\frac{1}{2}\left\Vert \left[\begin{array}{c}
\mat\left(\T{A}_{2}^{\top},\T{A}_{1}^{\top}\right)\\
\sqrt{\frac{\mu}{\lambda}} \M{I}_{n_2 n_3\cdot \ell}
\end{array}\right]\tvec\left(\T{A}_{3}^{\top}\right)-\left[\begin{array}{c}
\tvec\left(\T{X}^{\top}\right)\\
\sqrt{\frac{\mu}{\lambda}}\tvec\left(\T{H}_{3}^{\top}+\T{Y}_{3}^{\top}/\mu\right)
\end{array}\right]\right\Vert _{F}^{2},
\label{eq:ralsA3}
\end{equation}
where $\mat\left(\T{A}_{2}^{\top},\T{A}_{1}^{\top}\right)\in \mathbb{R}^{n_2 n_3\cdot n_1 \times n_2 n_3\cdot \ell}$.

%\begin{equation}
%\min_{\tvec\left(\T{A}_{1}^{\top^2}\right)}\frac{1}{2}\left\Vert \left[\begin{array}{c}
%\mat\left(\T{A}_{3}^{\top^2},\T{A}_{2}^{\top^2}\right)\\
%\sqrt{\frac{\mu}{\lambda}} \M{I}_{n_3 n_1\cdot 
%\ell}
%\end{array}\right]\tvec\left(\T{A}_{1}^{\top^2}\right)-\left[\begin{array}{c}
%\tvec\left(\T{X}^{\top^2}\right)\\
%\sqrt{\frac{\mu}{\lambda}}\tvec\left(\T{H}_{1}^{\top^2}+\T{Y}_{1}^{\top^2}/\mu\right)
%\end{array}\right]\right\Vert _{F}^{2},
%\label{eq:ralsA1}
%\end{equation}
%where $\mat\left(\T{A}_{3}^{\top^2},\T{A}_{2}^{\top^2}\right)\in \mathbb{R}^{n_3 n_1\cdot n_2 \times n_3 n_1\cdot 
%\ell}$.

\end{document}


